Pea-KD: Parameter-efficient and Accurate Knowledge Distillation on BERT

How can we efficiently compress a model while maintaining its performance? Knowledge Distillation (KD) is one of the widely known methods for model compression. In essence, KD trains a smaller student model based on a larger teacher model and tries to retain the teacher model's level of performance as much as possible. However, existing KD methods suffer from the following limitations. First, since the student model is smaller in absolute size, it inherently lacks model capacity. Second, the absence of an initial guide for the student model makes it difficult for the student to imitate the teacher model to its fullest. Conventional KD methods yield low performance due to these limitations. In this paper, we propose Pea-KD (Parameter-efficient and accurate Knowledge Distillation), a novel approach to KD. Pea-KD consists of two main parts: Shuffled Parameter Sharing (SPS) and Pretraining with Teacher's Predictions (PTP). Using this combination, we are capable of alleviating the KD's limitations. SPS is a new parameter sharing method that increases the student model capacity. PTP is a KD-specialized initialization method, which can act as a good initial guide for the student. When combined, this method yields a significant increase in student model's performance. Experiments conducted on BERT with different datasets and tasks show that the proposed approach improves the student model's performance by 4.4\% on average in four GLUE tasks, outperforming existing KD baselines by significant margins.

==> 100Intro.tex <==
\textit{How can we improve knowledge distillation (KD) accuracy with smaller number of parameters?}

KD uses a well-trained large teacher model to train a smaller student model. Conventional KD method (\cite{Hinton06}) trains the student model using the teacher model's predictions as targets. That is, the student model uses not only the true labels (hard distribution) but also the teacher model's predictions (soft distribution) as targets. Since better KD accuracy is directly linked to better model compression, improving KD accuracy is valuable and crucial.   

Naturally, there have been many studies and attempts to improve upon KD performance. \cite{sun2019patient} introduced Patient KD which utilizes not only the teacher model's final output but also the intermediate outputs generated from the teacher's layers. \cite{jiao2019tinybert} applied additional KD in the pretraining step of the student model. However existing KD methods share the limitation of students having lower model complexity compared to their teacher models, since they are small in size. In addition, there are no proper initial guides for the student model, which is important especially when the student models are small. These limitations result in modest performance.

In this paper, we propose Parameter-efficient and Accurate Knowledge Distillation (PeA-KD), a novel KD method especially for Transformer-based models (\cite{vaswani2017attention}), which significantly improves the student model's accuracy.
PeA-KD is composed of two methods, Shuffled Parameter Sharing (SPS) and Pretraining with Teacher's Predictions (PTP). These two methods combined alleviate the aforementioned KD's limitations and yield higher performance. PeA-KD is based on the following two main ideas.
\begin{itemize}
	\item[1.] We apply SPS in order to increase the effective model complexity of the student model while keeping the  number of parameters constant. SPS has two steps: 1) first stacking the layers that share parameters, and 2) shuffling the parameters between shared pairs of layers. Doing so increases the model's effective complexity which enables the student to better replicate the teacher model (details in Section \ref{320SPS}).
	\item[2.] We designed an artificial pretraining task called PTP. Through PTP, the student model can obtain additional information about the teacher and the task itself, which helps the student acquire the teacher's knowledge more efficiently during the KD process (details in Section \ref{330PTP}).  
\end{itemize} 
Throughout the paper we use \Method (Parameter-efficient and accurate BERT), which is PeA-KD applied on BERT, as an example to investigate our proposed approach. We summarize our main contributions as follows: 
\begin{itemize}
	\item \textbf{Novel framework for KD.} We propose SPS and PTP, a novel parameter sharing method and a novel KD-specialized initialization method. These methods can serve as a new framework for KD to significantly improve performance. 
	\item \textbf{Performance.} When tested on four of the widely used GLUE tasks, \Method improves KD accuracy up to 14.8\% and 4.4\% on average compared to the original BERT model. \Method also outperforms the existing state-of-the-art KD baselines by 3.4\% on average.
	\item \textbf{Generality.} 
	Our proposed method PeA-KD can be applied to any transformer-based models and any classfication tasks with minimal  modification. Our method can thus be generally applied to most ongoing KD studies in Natural Language Processing.	
\end{itemize}The rest of the paper is organized as follows. Section 2 covers related works. Section 3 describes our proposed method in detail. Section 4 presents experimental results. Then we conclude in section 5.


==> 200Related.tex <==
\paragraph{Pretrained Language Models.}
The framework of first pre-training language models and then finetuning for downstream tasks has now become the industry standard for Natural Language Processing (NLP) models. Pre-trained language models, such as BERT (\cite{devlin2018bert}), XLNet (\cite{yang2019xlnet}), RoBERTa (\cite{liu2019roberta}) and ELMo (\cite{peters2018deep}) prove how powerful pretrained language models can be. Specifically, BERT is a language model consisting of multiple Transformer layers. By pretraining using Masked Language Modeling (MLM) and Next Sentence Prediction (NSP), BERT has achieved state-of-the-art performance on a wide range of NLP tasks, such as the GLUE benchmark (Wang et al., 2018) and SQuAD (Rajpurkar et al., 2016). However, these modern pretrained models are very large in size and contain millions of parameters, making them nearly impossible to apply on edge devices with limited amount of resources. In our work, we address this challenging problem by applying novel KD method on the BERT model. Our approach can be easily applied to other transformer-based models as well.

\paragraph{Model Compression.}

As deep learning algorithms started getting adopted, implemented, and researched by diverse fields, high computation costs and memory shortage have started to become challenging factors. Especially in NLP, pretrained language models typically require a large set of parameters. This results in extensive cost of computation and memory. As such, Model Compression, which is compressing a model while preserving the performance as much as possible, has now become an important task for deep learning. There have already been many attempts to tackle this problem, including quantization (\cite{gong2014compressing}) and weight pruning (\cite{han2015learning}). One promising approach is KD  (\cite{hinton2015distilling}) which we will focus on in this paper.

\paragraph{Knowledge Distillation.} 
As briefly covered in Section \ref{100Intro}, KD transfers knowledge from a well-trained and large teacher model to a smaller student model. KD uses the teacher model’s predictions on top of the true labels to train the student model. It is proven through many experiments that the student model learns to imitate the soft distribution of the teacher model’s predictions, and ultimately performs better than learning solely from the original data. 
There have already been many attempts to compress BERT using KD. Patient Knowledge Distillation (\cite{sun2019patient}) extracts knowledge not only from the final prediction of the teacher, but also from the intermediate layers. TinyBERT (\cite{jiao2019tinybert}) uses a two-stage learning framework which applies knowledge distillation in both pretraining and task-specific finetuning. DistilBERT (\cite{sanh2019distilbert}) uses half of the layers of BERT-base model and applies KD during pretraining and finetuning of BERT. \cite{zhao2019extreme} trains the student model with smaller vocabulary set and lower hidden state dimensions. Despite the recent progress in research, these existing methods yield modest performance due to the student model's insufficient complexity and absence of a clear guideline for initialization.
In our paper, we propose a new KD approach to better transfer knowledge from the teacher to the student improving the student model's performance significantly. Our method shows the state-of-the-art performance among distillation methods on BERT. 
\paragraph{Parameter Sharing.}
The idea of parameter sharing across different layers is a widely used idea for model compression. There have been several attempts to use parameter sharing in transformer architecture and BERT model. However, existing parameter sharing methods exhibit high tradeoff between model performance and model size. It can reduce the model's size significantly but as a result, also suffers in great loss in performance. In our paper, we propose a novel parameter sharing method which uses a shuffling mechanism to reduce this tradeoff, resulting in improved performance using the same number of parameters.


==> 300Method.tex <==
We propose \Method, a novel KD baseline applied on BERT that shows higher KD accuracy with small number of parameters. \Method consists of two main ideas: SPS and PTP, which together boost the student model's performance. 
In the sections that follow, we provide an overview of the main challenges in KD and our methods to address them in Section \ref{310Overview}. We then discuss the precise procedures of SPS and PTP in sections \ref{320SPS} and \ref{330PTP}. Lastly, we explain our final method, \Method and the training details in Section \ref{340KDAPP}.
\subsection{Overview}
\label{310Overview}
The BERT-base model contains over 109 million parameters. Its extensive size makes model deployment often infeasible and computationally expensive in many cases, such as model deployment on mobile devices. As a result, industry practitioners commonly use a smaller version of BERT and apply KD. However, the existing KD methods entail the following challenges: 
\begin{itemize}
	\item \textbf{Insufficient model complexity of student model.} Since the student model contains fewer number of parameters than the teacher model, it's model complexity is also lower. The smaller and simpler the student model gets, the gap between the student and the teacher grows, making it increasingly difficult for the student to replicate the teacher model's performance. The limited complexity hinders the student model's performance. How can we enlarge the student model's complexity while maintaining the same number of parameters? 
	\item \textbf{Absence of proper initial guide for the student model.} Most of the existing KD methods do not consider the student model's initialization to be crucial. In most cases, a  truncated version of pretrained BERT-base model is used. There is no widely accepted and vetted guide to selecting the student's initial state of the KD process. In reality, this hinders the student from efficiently reproducing the teacher's results. How can we effectively initialize the student model to achieve a better KD accuracy? 
	%\item \textbf{Gap between the student and teacher model.} As we use smaller models for student model, the gap between the student and teacher increases and makes it harder for the student to imitate the teacher model's outputs. 
\end{itemize}

We propose the following main ideas to address the challenges:

\begin{itemize}
	\item \textbf{SPS: Amplifying 'effective' model complexity of the student.} To address the complexity limitation, we introduce SPS. SPS increases the student's 'effective' model complexity while using the same number of parameters (See details in Section \ref{320SPS}). As a result, the SPS-applied student model can achieve better performance without running into the usual computational challenges. 
	\item \textbf{PTP: Novel pretraining task utilizing teacher's predictions for student initialization.} To address the initial guide limitation, we propose PTP, a novel pretraining with teacher model's predictions. Through PTP, the student model can pre-learn information about the teacher and the task itself. It helps the student better acquire the teacher's knowledge during the KD process (See details in Section \ref{330PTP}). 
\end{itemize}
The following sections describe the precise procedures of SPS, PTP, and \Method in detail.

\subsection{Shuffled Parameter Sharing (SPS)}
\label{320SPS}
\begin{figure}[h]
	\centering
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=1.0\linewidth]{FIG/Figure1_a}
		\caption{SPS step 1}
		\label{fig:SPS_a}
	\end{subfigure}
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=1.0\linewidth]{FIG/Figure1_b}
		\caption{SPS step 1 + step 2}
		\label{fig:SPS_b}
	\end{subfigure}
	\begin{subfigure}{0.3\textwidth}
		\includegraphics[width=1.0\linewidth]{FIG/Figure1_c}
		\caption{SPS for six-layer student}
		\label{fig:SPS-6}
	\end{subfigure}
	\caption{Graphical representation of SPS: (a) the first step of SPS, (b) the second step of SPS, and (c) modified SPS for six layer student student. }
	\label{fig:SPS}
\end{figure}
SPS improves student's effective model complexity while keeping the number of parameters constant, addressing the complexity limitations typical of KD. SPS is composed of two steps.

\textbf{Step1. Paired Parameter Sharing.}
We start with doubling the number of layers in the student model. We then share the parameters between the bottom half and the upper half of the model, as graphically represented in Figure \ref{fig:SPS_a}. By doing so the model now has twice the number of layers and thus higher effective model complexity while maintaining the same number of actual parameters used.
 
\textbf{Step2. Shuffling.}
We shuffle the Query and Key parameters between the shared pairs. This allows the parameter shared pairs to have more degree of freedom and behave closely to individual layers, resulting in increased model complexity of the student. We will call this architecture SPS, which is depicted in Figure \ref{fig:SPS_b}. For the 6-layer student case we slightly modify the architecture as in Figure \ref{fig:SPS-6} (we apply SPS on the top 3 layers only).

In sum, the SPS model has the same number of parameters as the original student model but has much greater effective model complexity, if not double. In later section, we will validate through experiments that step1 (Paired Parameter Sharing) and step2 (Shuffling) indeed increase the effective model complexity, directly attributing to performance improvement.
\subsection{Pretraining with Teacher's Predictions (PTP)}
\label{330PTP}
There can be several candidates for KD-specialized initialization. We propose a pretraining approach called PTP, and will prove that it improves KD accuracy significantly via experiments. The intuition here is that by undergoing PTP, the student model pretrains and acquires additional knowledge about both the teacher as well as the downstream task. With this additional information, the student obtains the teacher's knowledge more efficiently during the actual KD process. 

Most of the previous studies done regarding KD did not elaborate on the initialization of the student model. There are some studies that used pretrained student model as the initial state, but those pretraining tasks were irrelevant to either the teacher model or the downstream task. To the best of our knowledge, our study is the first case that pretrains the student model with a task relevant to the teacher model and downstream task. PTP consists of two steps:   

\textbf{Step 1. Creating artificial data based on the teacher's predictions (PTP labels).}

We first input the training data in the teacher model and collect the teacher model's predictions. We then define "confidence" as the following. We apply softmax function to the teacher model's predictions, and the maximum value of the predictions is defined as the confidence. Next, with a specific threshold "t" (a hyperparameter between 0.5 and 1.0), we assign a new label to the training data according to the rules cited in table \ref{table:new label}. We will call these new artificial labels PTP labels.
\begin{table}[h]
	\caption{Assigning new PTP labels to the training data.}
	\label{sample-table}
	\centering
	\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lcc}
		\toprule
		%\hline
		% %\multicolumn{1}{c}{} &\multicolumn{4}{c}{methods}    \\
		
		PTP label & Teacher's prediction correct   & confidence $>$ t   \\
		\midrule
		confidently correct & True & True   \\
		unconfidently correct & True     & False        \\
		confidently wrong & False    & True    \\
		unconfidently wrong & False  & False  \\
		\bottomrule
		
	\end{tabular*}
	\label{table:new label}
\end{table}

\textbf{Step 2. Pretrain the student model to predict the PTP labels.}
Using the artificial PTP labels (data $x$, PTP label) we created, we can now pretrain the student model to predict the PTP label when data $x$ is provided as input. In other words, the student model is trained to predict the PTP labels given the downstream training dataset. We train the student model until convergence.   

Once these two steps are complete, we can now use this PTP pretrained student model as the initial state for finetuning on the downstream task. 
\subsection{\Method: SPS and PTP combined}
\label{340KDAPP}
\subsubsection{overall details of \Method}
Our complete \Method applies SPS and PTP together on BERT for maximum impact on performance. That is, given a student model, we first transform it into an SPS model and apply PTP. Once PTP is complete, we use this model as the initial state of the student model during the KD process. The overall framework of \Method is depicted in Figure \ref{fig:PTP}.
\begin{figure}[h]
	\centering
	\ %begin{subfigure}{0.45\textwidth}
	\includegraphics[width=1.0\linewidth]{FIG/Figure2}
	%\end{subfigure}
	\caption{The overall framework of \Method. Left half represents applying SPS and PTP to student model. Right half represents the learning baseline.}
	\label{fig:PTP}
\end{figure}
\subsubsection{Learning details of \Method}
For the starting point of the KD process, a well finetuned teacher model should be used. To study the effectiveness of our proposed \Method model, we use a 12 layer BERT-base model as the teacher. The learned parameters are denoted as:
\begin{equation}
	\centering
	\hat{\theta}^{t} = \argmin\limits_{\theta^{t}}\sum\limits_{i \in N}\mathcal{L}_{CE}(y_{i}, \sigma(z_{t}(x_{i}; \theta^{t})))
\end{equation}
where the $\theta^{t}$ denotes parameters of the teacher, $\sigma$ denotes the softmax function, $x_{i}$ denotes the training data, $z_{t}$ denotes the teacher model's output predictions, $y_{i}$ denotes the true labels, and $\mathcal{L}$$_{CE}$ denotes cross-entropy loss.
We then pretrain the student model with PTP labels using the following equation:
\begin{equation}
	\centering
	\hat{\theta}^{s}_{_{\mathcal{PTP}}} = \argmin\limits_{\theta^{s}}\sum\limits_{i \in N}\mathcal{L}_{CE}(y^{\mathcal{PTP}}_{i}, \sigma(z_{s}(x_{i}; \theta^{s})))
\end{equation}
where, $y^{\mathcal{PTP}}_i$ denotes the PTP labels and the subscript $s$ denotes the student model. When PTP is complete, we use the $\hat{\theta}^{s}_{_{\mathcal{PTP}}}$ as the initial state of the KD process. During the KD process, we used a softmax-temperature T which controls the softness of teacher model's output predictions (\cite{hinton2015distilling}):
\begin{equation}
\centering
\sigma_{T}(z_{i}) = {e^{z_{i}/T} \over \sum\limits_{j}e^{z_{j}/T}}  
\end{equation}

The loss function is as follows:
\begin{equation}
	\centering
	\mathcal{L} =  \alpha\mathcal{L_{KL}}(\sigma(z_{s}(x_{i};\theta^{s}),\sigma_{T}(z_{t}(x_{i};\hat{\theta^{t}})))) + (1-\alpha)\mathcal{L}_{CE}(y_{i}, \sigma(z_{s}(x_{i};\theta^{s})) + \beta\sum\limits_{k \in \mathcal{K}}||z^{k}_{s} -z^{k}_{t}||^{2}_{2}
\end{equation}
where $\mathcal{L_{KL}}$ denotes the Kullback-Leibler divergence loss, $\mathcal{K}$ denotes the indices of particular layers we use in Patient KD, and $z^{k}$ denotes the output logits of the k-th layer. $\alpha$ and $\beta$ are hyperparameters. 


==> 400Experiments.tex <==
In this section, we will discuss the experiments we performed to assess the effectiveness of our proposed method. Our goal was to answer the following questions.
\begin{itemize}
	\item{\textbf{Q1.}} \textbf{Overall Performance.} How does \Method perform compared to the currently existing KD methods? (Section \ref{420Overall_Performance})
	\item{\textbf{Q2.}} \textbf{Effectiveness of SPS.} To what extent does the SPS process improve the effective complexity of the student model? (Section \ref{430SPS_Effect})
	\item{\textbf{Q3.}} \textbf{Effectiveness of PTP.} Is the new PTP-training a good initialization method? Compared to the conventionally used truncated version of the BERT-base model, what is the impact that our PTP initialization method has on model performance?(Section \ref{440PTP_Effect})
\end{itemize} 
\subsection{Experimental Settings and Datasets Used}
\textbf{Datasets.} We evaluate our proposed methods on four of the most widely used datasets in the General Language Understanding Evaluation (GLUE) benchmark (\cite{wang2018glue}): SST-2\footnote{https://nlp.stanford.edu/sentiment/index.html}, QNLI\footnote{https://rajpurkar.github.io/SQuAD-explorer/}, RTE\footnote{https://aclweb.org/aclwiki/RecognizingTextualEntailment}, and MRPC\footnote{https://www.microsoft.com/en-us/download/details.aspx?id=52398}. For sentiment classification, we use the Stanford Sentiment Treebank (SST-2) (\cite{socher2013recursive}). For natural language inference, we use QNLI(\cite{rajpurkar2016squad}) and RTE. For paraphrase similarity matching, we use Microsoft Research Paraphrase Corpus (MRPC) (\cite{dolan2005automatically}). Specifically, SST-2 is a movie review dataset with binary annotations where the binary label indicates positive and negative reviews. QNLI is a task for predicting whether a pair of question and answer is entailment or not. RTE is based on a series of textual entailment challenges and MRPC contains pairs of sentences and corresponding labels, which indicate the semantic equivalence relationship between each pair.  

\textbf{Competitors.}
We use Patient Knowledge Distillation (PKD, \cite{sun2019patient}) as our baseline learning method to compare and quantify the effectiveness of our proposed approach. Patient Knowledge Distillation is a variant of original Knowledge Distillation method (\cite{Hinton06}) which is one of the most widely used baselines. We conduct our experiments on BERT model (\cite{devlin2018bert}) and compare the results of \Method to the original BERT. In addition, we compare the results with other state-of-the-art BERT-distillation models, including DistillBERT(\cite{sanh2019distilbert}) and TinyBERT(\cite{jiao2019tinybert}).

\textbf{Training Details.}
We use the full twelve-layer original BERT model (\cite{devlin2018bert}) as the teacher model and further finetune the teacher for each task independently. The student models are created using the same architecture as the original BERT, but the number of layers were reduced to either 1,2,3, and 6 layers depending on the experiment. That is, we initialize the student model using the first n-layers of parameters from the pretrained original BERT obtained form Google's official BERT repo\footnote{https://github.com/google-research/bert}.
Industry norms are used to create the baseline to measure the effectiveness of our proposed method. PKD is used, and the following hyperparameter settings are used. Training batch size is chosen from \{32, 64\}, learning rate from \{1, 2, 5\}$\cdot10^{-5}$, and number of epochs from \{6, 10\}. 
\subsection{Overall Performance}
\label{420Overall_Performance}
\begin{table}[t]
	\centering
	\caption{Overall results of \Method compared to the state-of-the-art KD baseline, PKD. The results are evaluated on the test set of GLUE official benchmark. The subscript numbers denote the number of independent layers of the student. F1 metric is used for MRPC.}
	\label{tab:overall}
	%\begin{adjustbox}{width=0.7 \textwidth}
	\begin{adjustbox}{width=1 \textwidth}
		\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lccccc}
			\toprule
			
			Method &  RTE & MRPC & SST-2 & QNLI & Avg\\
			
			\midrule
			BERT$_{1}$-PKD & 52.8 & 80.6 & 83.6 & 64.0 & 70.3\\
			
			PeaBERT$_{1}$ & 53.0 & 81.0 & 86.9 & 78.8 & 75.0  \\
			
			\midrule
			
			BERT$_{2}$-PKD & 53.5 & 80.4 & 87.0 & 80.1 & 75.2 \\
			
			PeaBERT$_{2}$ & 64.1 & 82.7 & 88.2 & 86.0 & 80.3  \\
			
			\midrule
			
			BERT$_{3}$-PKD & 58.4 & 81.9 & 88.4 & 85.0 & 78.4 \\
			
			PeaBERT$_{3}$  & 64.5 & 85.0 & 90.4 & 87.0 & 81.7 \\
			
			\bottomrule	
		\end{tabular*}
		
	\end{adjustbox}
	%\end{adjustbox}
\end{table}				

\begin{table}[t]
	\centering
	\caption{\Method in comparison to other state-of-the-art competitors in dev set. The cited results of the competitors are from the official papers of each method. For accurate comparison, model dimensions are fixed to six layers across all models compared.}
	\label{tab:overall_2}
	%		\begin{adjustbox}{width=1.0 \textwidth}
	\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lcccccc}
		\toprule
		
		Method & \# of parameters & RTE & MRPC & SST-2 & QNLI & Avg \\
		
		\midrule
		
		%BERT$_{6}$-PKD   & 42.6M  & - & - & - & - & - \\
		
		DistillBERT   & 42.6M  & 59.9 & 87.5 & 91.3 & 89.2 & 82.0    \\
		
		TinyBERT   & 42.6M  & 70.4 & 90.6 & 93.0 & 91.1 & 86.3   \\
		
		\midrule
		
		\Method     & 42.6M   & 73.6  & 92.9 & 93.0 & 90.3 & 87.5 \\
		\bottomrule	
	\end{tabular*}
\end{table}		
We summarize the performance of our proposed method, \Method, against the baseline in Table \ref{tab:overall}. We also compare the results of \Method against its competitors DistilBERT and TinyBERT in table \ref{tab:overall_2}. We observe the following from the results.
	
First, we see from Table \ref{tab:overall} that \Method consistently yields higher performance in downstream tasks across all three model sizes that were tested. Notably, the proposed method shows average improvements of 4.7 points for the 1-layer student, 5.1 points for the 2-layer student, and 3.3 points for the 3-layer student. These results strongly validate the effectiveness of our proposed PeA-KD framework across varying downstream tasks and student model sizes. 
	
Second, using the same number of parameters, \Method outperforms the state-of-the-art KD baselines DistilBERT and TinyBERT, by 5.5\% and 1.2\% on average. We use a 6-layer student model for this comparison. An inspiring advantage of \Method is that it achieves remarkable performance improvement just by using the downstream dataset without touching the original pretraining tasks. Unlike its competitors, \Method does not touch the original pretraining tasks. Specifically, Masked Language Modeling (MLM) and Next Sentence Prediction (NSP). This reduces training time significantly. For example, DistilBERT took approximately 90 hours with eight 16GB V100 GPUs while \Method took a minimum of one minute (PeaBERT$_{1}$ with RTE) to a maximum of one hour (PeaBERT$_{3}$ with QNLI) using just two NVIDIA T4 GPUS.     
	
Finally, another strong suit of \Method is that it can be directly applied to other transformer-based models with minimal modificiations. The SPS method can be directly applied to any transformer-based models, and the PTP method can be applied to any classification task. For instance, we can easily implement the proposed method on DistilBERT and TinyBERT models, which will likely further improve their performance. 

\subsection{Effectiveness of SPS}
\label{430SPS_Effect}
\begin{table}[h!]
	%\vspace*{-30pt}
	\centering
	\caption{An ablation study to validate each steps of SPS. A three-layer student model is chosen as representative. The results are derived using GLUE dev set.}
	% %\label{sample-table}
	\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lcccccc}
		\toprule
		Method 	 &\# of parameters & RTE    & MRPC   & SST-2 & QNLI   & Avg \\
		\midrule
		BERT$_{3}$  & 21.3M   & 61.4  & 84.3  &  89.4     & 84.8  & 80.0 \\
		SPS-1  & 21.3M   & 63.5  & 85.8  &  89.6     &  85.5     & 81.1 \\
		SPS-2  & 21.3M   & 68.6  & 86.8  & 90.2     & 86.5  & 83.0 \\
		\bottomrule
	\end{tabular*}
	\label{tab:Ablation_SPS}
\end{table}
In this section we perform an ablation study to verify the effectiveness of SPS at increasing the student model's complexity. We compare three models BERT$_{3}$, SPS-1, and SPS-2. BERT$_{3}$ is the original BERT model, which applies none of the SPS steps. As such, this is used as the baseline for comparison. SPS-1 applies only the first step in the SPS process to BERT$_{3}$. SPS-2 applies both the first and second SPS steps to BERT$_{3}$. 

The ablation study is conducted on BERT$_{3}$ as a representative model and the results are summarized in table \ref{tab:Ablation_SPS}. Compared to the original BERT$_{3}$, SPS-1 shows improved accuracy in all the downstream datasets with an average of 1.1 points. Comparing SPS-1 with SPS-2, we note that SPS-2 consistently shows better performance with an average of 1.9 points. We can therefore conclude that both steps of the SPS process individually increase the effective model complexity of student model. 

\subsection{Effectiveness of PTP}
\label{440PTP_Effect}
\begin{table}[h]
	\centering
	\caption{An ablation study to verify the effectiveness of PTP. The results are derived using GLUE dev set.}
	\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}lcccccc}
		\toprule
		Model & \# of parameters &RTE & MRPC  & SST-2 & QNLI & Avg    \\
		\midrule
		PeaBERT$_{3}$-p & 21.3M   & 68.6 & 86.8 & 90.2 & 86.5 & 82.9 \\
		PeaBERT$_{3}$ & 21.3M    & 70.8 & 88.0 & 91.2 & 87.1  & 84.3\\
		
		\bottomrule		
	\end{tabular*}
	\label{tab:Ablation_PTP}
\end{table}
In this section, we perform an ablation study to validate the effectiveness of using PTP as an initial guide for the student model. Similarly to how we validate the effectiveness of SPS in section \ref{430SPS_Effect}, we use BERT$_{3}$ as our representative model and compare PeaBERT$_{3}$ to its variant PeaBERT$_{3}$-p. PeaBERT$_{3}$-p is the \Method model without PTP. This essentially is applying only SPS to BERT$_{3}$. PeaBERT$_{3}$ goes one step further and applies both SPS and PTP. The results are reported in Table \ref{tab:Ablation_PTP}.

As summarized in Table \ref{tab:Ablation_PTP}, applying PTP increases accuracy across all four of the datasets with an average of 1.4 points, proving the effectiveness of using PTP to increase model performance. We can now validate our second main claim that initializing a student model with KD-specialized initialization prior to applying KD improves performance. As existing KD methods do not place much emphasis on the initialization process, this finding highlights a potentially major, undiscovered path to improving model performance. Further and deeper research related to KD-specialized initialization could be promising.

==> 500Conclusion.tex <==
In this paper, we introduced and proved the efficacy of a new KD method for transformer-based distillation, PeA-KD. Our goal was to address and reduce the limitations of the currently available KD methods. We first introduced SPS, a new parameter sharing approach that uses shuffling mechanism, which enhances the complexity of the student model while using the same number of parameters. We then introduced PTP, a KD-specific initialization method for the student model. Applying these two methods on BERT, we introduced \Method. Through experiments conducted using multiple datasets and varying model sizes, we showed that our method improves KD accuracy significantly. We showed that \Method works well across different datasets and outperforms the original BERT as well as other state-of-the-art baselines on BERT distillation. 
 
In future work, we would like to delve deeper into the concept of KD-specialized initialization of the student model. Also, since PTP and SPS are independent processes on their own, we anticipate model compression to further improve when combined with other existing model compression techniques, such as weight pruning and quantization. 

